Vector-ICL: In-context Learning with Continuous Vector Representations

Large language models (LLMs) have shown remarkable in-context learning (ICL) capabilities on textual data. We explore whether these capabilities can be extended to continuous vectors from diverse domains, obtained from black-box pretrained encoders. By aligning input data with an LLM's embedding space through lightweight projectors, we observe that LLMs can effectively process and learn from these projected vectors, which we term Vector-ICL. In particular, we find that pretraining projectors with general language modeling objectives enables Vector-ICL, while task-specific finetuning further enhances performance. In our experiments across various tasks and modalities, including text reconstruction, numerical function regression, text classification, summarization, molecule captioning, time-series classification, graph classification, and fMRI decoding, Vector-ICL often surpasses both few-shot ICL and domain-specific model or tuning. We further conduct analyses and case studies, indicating the potential of LLMs to process vector representations beyond traditional token-based paradigms.

==> tex/figures/analysis_encoder.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth, keepaspectratio]{img/encoder_analysis.pdf}
    \caption{\textbf{Case studies} }
    \label{fig:encoder_analysis}
\end{figure}

==> tex/figures/main_results_figure_3by3.tex <==
% \begin{figure}[ht]
%     \centering
%     % First row
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/reconstruction_all.pdf}
%         \label{fig:reconstruction}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/math10_all.pdf}
%         \label{fig:math10}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/classification_all.pdf}
%         \label{fig:classification}
%     \end{subfigure}
    
%     % Second row
%     \vspace{-0.2cm}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/summarization_all.pdf}
%         \label{fig:summarization}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/molecule_all.pdf}
%         \label{fig:molecule}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/braintext_all.pdf}
%         \label{fig:braintext}
%     \end{subfigure}
    
%     % Third row
%     \vspace{-0.2cm}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/brainclassification_all.pdf}
%         \label{fig:brainclassification}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/timeseries_all.pdf}
%         \label{fig:timeseries}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[height=4.3cm]{img/graph_all.pdf}
%         \label{fig:graph}
%     \end{subfigure}
    
%     \caption{Main Results for Different Tasks}
%     \label{fig:main_results}
% \end{figure}

==> tex/s3.5_setup_backup.tex <==
% We utilize four state-of-the-art LLMs in our experiments: Meta-Llama-3.1-8B-Instruct~\citep{dubey2024llama3},  Mistral-7B-Instruct-v0.3~\citep{jiang2023mistral}, Qwen2-7B-Instruct~\citep{yang2024qwen2}, and Yi-1.5-9B-Chat~\citep{young2024yi}.

% we provide detailed explanations for each task, including the encoders used for constructing embeddings, the datasets employed, the formulation of task-specific prompts, and the placement of the projected embeddings within those prompts. 
% A summary of these details is provided in~\cref{tab:setup}.

% In addition, we denote the subset in task prompts involved in the conditional generation loss during projector finetuning with underlines, for example: $x=\Box_x$, $x$  equals to (digits): \underline{128}.

% \input{tex/tables/main_task_table}

\paragraph{General NLP Task and Text Pretraining} 
For our NLP tasks, We employ four encoders that are highly ranked on the MTEB benchmark~\citep{muennighoff2022mteb}: NV-Embed-v1~\citep{lee2024nvembed}, SFR-Embedding-2R~\citep{meng2024sfrembedding}, stella-en-1.5B-v5~\citep{stella-en-v5} and gtr-t5-base~\citep{ni2021gtr}.
These encoders are used for all textual inputs including the molecule chemical sequences.

We use WikiText-103~\citep{merity2016wikitext} dataset to pretrain our text projectors. 
It is a collection of over 100 million tokens extracted from the set of verified Good and Featured articles on Wikipedia.
We chose this smaller language modeling corpus because the projector is lightweight and small in parameter scale.

The pretraining process is illustrated in~\cref{fig:pipeline_train}(a). 
We uniformly sample a separation point for each text snippet from the end of sentences.
The first half is embedded and projected, while a next-token generation loss is applied to the second half.

\paragraph{Text Reconstruction}
We use two datasets for the text reconstruction task, Parallel Sentence Talks's English subset~\citep{tiedemann2012parallelsetence} and Quora~\citep{thakur2021beir}.

Parallel Sentence Talks consist of sentences used in movie conversations, and Quora is built on a wide range of online questions.
They represent short pieces of text that convey clear information. 
We aim to explore whether LLMs can decode the original message from the projected text embeddings.

We use the following prompt template:

\makebox[\textwidth]{Translate the text in brackets: $(\Box)$, translation: \underline{[Original Text]}}

We train the projectors on the training set of these two datasets and evaluate their performance on the test tests.
We measure the reconstruction performance with the BLEU score~\citep{papineni2002bleu, sacrebleu}.

\paragraph{Arithmetic and Function Regression}
We created synthetic datasets of numerical data to pretrain our linear number projectors, experimenting with two configurations: one using 3-digit numbers and the other using 10-digit numbers. In Llama3.1-8B’s tokenizer, 3-digit numbers are represented as single tokens, while in Mistral-7B, Qwen2-7B, and Yi-1.5-9B, numbers larger than 10 are split into multiple tokens. Consequently, 10-digit numbers consistently span multiple tokens across all models, which increases the complexity of performing arithmetic operations.

To represent the numbers, we use a concatenated-and-flattened one-hot vector encoding for each digit. 
For instance, a 3-digit number is represented as a $3 \times 10$ matrix (one hot per digit place), which is then flattened into a 30-dimensional vector. 
Similarly, a 10-digit number is represented as a $10 \times 10$ matrix, flattened into a 100-dimensional vector.

The pretraining involves two tasks. 
The first task is number reconstruction, we use the following prompt template, given the number is 128:

\makebox[\textwidth]{$x=\Box_x$,\quad $x$  equals to (digits): \underline{128}}

The second task is basic addition, we use the following prompt template, given the numbers are $x=128\;y=256,\;a=1,\;b=1$:

\makebox[\textwidth]{$x=\Box_x,\; y=\Box_y$,\quad $a*x+b*y$ equals to (digits): \underline{384}}

Here, $a$ and $b$ are randomly sampled from $[0,1]$ with up to two decimal places, and the solution is the integer part of the sum.

For evaluation, we use a function regression task with a non-linear function: $f(x, y) = \sqrt{x} \cdot \sqrt{y}$. 
The LLM is given inputs $x$ and $y$, along with the integer part of the output $f(x, y)$. 
The model is then tasked with predicting the output for new pairs of $x$ and $y$. 
The prompt for in-context learning is structured as follows:

\makebox[\textwidth]{$x=\Box_x,\; y=\Box_y$,\quad function($x, y$) equals to (digits): \underline{[Solution]}}

For few-shot ICL, the box tokens will be replaced with the actual numbers.
We measure the function regression performance with the mean relative error, where the relative error is computed as the $\ell_1$ difference divided by the ground truth value.

\paragraph{Text Classification}
We use five datasets for the text classification task. 
For binary classification, we include IMDB~\citep{maas-EtAl:2011:IMDB}, Rotten Tomatoes~\citep{Pang+Lee:05a:rotten_tomatoes}, and the Stanford Sentiment Treebank (SST2)~\citep{socher-etal-2013-sst2}. 
For multi-class classification, we use the Emotion dataset~\citep{saravia-etal-2018-emotion} and the Financial Phrasebank~\citep{Malo2014financial_phrasebank}.
The binary classification datasets (IMDB, Rotten Tomatoes, and SST2) involve classifying movie reviews as positive or negative. 
The Emotion dataset classifies Twitter tweets into six categories: anger, fear, joy, love, sadness, and surprise. 
The Financial Phrasebank categorizes financial news into positive, negative, or neutral sentiments.

We use the following prompt in ICL:

\makebox[\textwidth]{$(\Box)$'s sentiment is \underline{[Input Class]}}

For few-shot ICL, the box tokens will be replaced with the actual text. For soft prompt tuning, we use 20 virtual tokens and train for one epoch over the entire training set.
We measure the classification performance with accuracy on the test set.


\paragraph{Text Summarization}
We use two datasets for the summarization task, XSum~\citep{Narayan2018xsum} and the English subset of XLSum~\citep{hasan-etal-2021-xlsum}.
They contain newspaper articles and their summaries.

We use the following prompt in ICL:

\makebox[\textwidth]{$(\Box)$'s summarization is: \underline{[Summary of the Input]}}

For few-shot ICL, the box token will be replaced by the article. 
We measure the performance using the RougeL score with the ground truth summary on the test sets.

\paragraph{Molecule Captioning}
We use the Language + Molecules-24 (LPM24) dataset for the molecule captioning task, it was created for the task of molecule-language translation, contains 161K pairs of molecule strings and their captions in the combined training and test set.

A sample molecule-caption pair looks like the following: 

\makebox[\textwidth][c]{
    \parbox{.9\textwidth}{
    Molecule: Cc1c(Cl)cccc1-n1ccn2c(SCC(=O)c3ccccc3C(F)(F)F)nnc2c1=O\\
    Caption: The molecule is a pain treatment that impacts inflammatory disease treatment.
    }
}

And we use the following prompt for ICL:

\makebox[\textwidth]{$(\Box)$'s molecule caption is: \underline{[Caption of the Input Molecule]}}

For few-shot ICL, we replace the box token with the actual molecule string.
We measure the performance using the BLEU score between the generated caption and the ground truth caption.


\paragraph{Brain fMRI Decoding and Classification}
We analyze data from \citeauthor{lebel2022natural}~\citeyear{lebel2022natural} and \citeauthor{tang2023semantic}~\citeyear{tang2023semantic}, which consists of fMRI responses for 3 human subjects as they listen to 20+ hours of narrative stories from podcasts.
We preprocessed the data following \citeauthor{benara2024crafting}~\citeyear{benara2024crafting}, by converting the fMRI responses into a 200-dimensional output using principal components analysis and labeling 10-grams of the story text at 2-second intervals using an ensemble of LLMs.

The data was separated into train set and test set by holding out the same three podcast stories from the three human subjects.
We use the same pretraining methodology as text to pretrain on the brain fMRI data. 
As the data comes in as segments of text and the recorded fMRI, we randomly sample 20\% of the segments to be in fMRI form and projected into box tokens, and we impose next token generation loss on the rest 80\%. 

We evaluate the projectors by giving them randomly sampled context from the train set, that could come from different human subject or from a different story, and ask them to decode segments from the test set.
We use the following prompt in ICL in our decoding experiments:

\makebox[\textwidth]{
    \parbox{0.75\textwidth}{
    What is the English translation of the input?\\ 
    Input: $\Box$, Response: the input in English is \underline{[Text Corresponding to fMRI]}}
}

The random baseline is constructed by giving LLM the randomly sampled, shuffled text from the training set, and generating text according to it.
We measure the performance using the RougeL score between the generated text and the ground truth.

We construct the classification questions around the properties of the underlying text, for example, ``Does the sentence contain a proper noun?'', ``"Does the input mention anything related to arguing?''.
The ground truth is obtained via GPT4o~\citep{openai2023gpt4} as binary labels.
We use the following prompt in ICL in our classification experiments, using one of the example questions:

\makebox[\textwidth]{
    \parbox{0.75\textwidth}{
    Does the input mention anything related to arguing?\\ 
    Input: $\Box$, Response (Yes or No): according to the English text of the input, the answer is \underline{[Yes/No]}}
}

The random baseline is 50\%, as we have downsampled and balanced the data. And we use accuracy as the performance metric.

\paragraph{Time-series}
We use the Chronos~\citep{ansari2024chronos} time-series Transformers as the encoder. 
Chronos was pretrained on large scale time-series and is designed to generate the next segments of the time-series.
It has proven effective on a wide range of time-series forecasting benchmarks. 
We take the output of the last time step from Chronos-base as the time-series representation.

We use two datasets for time-series classification, FordA, and FordB, they are both part of the UCR Time Series Classification Archive~\citep{dau2019ucrarchive} ranging from 4000 to 5000 time-series for each dataset.
We use the following prompt in ICL:

\makebox[\textwidth]{$(\Box)$'s class (positive, negative) is: \underline{[Input Class]}}

We use the base encoder with trained classification head as the baseline and we measure the prediction performance with accuracy.

\paragraph{Graphs}
We use Graphormer~\citep{ying2021graphormer} as the encoder model, specifically the one that was pretrained on large scale quantum chemistry graph datasets~\citep{hu2021ogb}.
Since the down-stream task (ogbg-molhiv~\citep{hu-etal-2020-ogbg}) is a molecule property prediction dataset, and with strong class imbalance (3\% positive classes), we finetune the encoder on the training set to provide meaningful baselines and embeddings.
We take the output prior to the classification layer of the Graphormer as the graph embedding.

We use the ogbg-molhiv~\citep{hu-etal-2020-ogbg} dataset for the graph classification task. 
ogbg-molhiv is a molecule property prediction dataset consisting of a total 41.12K graphs with node features and edge attributes.
It has a strong class imbalance of having around 3\% positive class and 97\% negative class.

Hence weighted sampling is adopted in the finetuning of both the baseline Graphormer and the embedding projector to yield meaningful predictions. 
We use the following prompt in ICL:

\makebox[\textwidth]{$(\Box)$'s class (positive, negative) is: \underline{[Input Class]}}

We use the finetuned Graphormer as our baseline and use the F1 score as the performance metric due to the significant class imbalance.

% \input{tex/tables/projector_task_table}
\paragraph{Projectors Configurations}
We have linear and non-linear projectors, and we used the configuration for each modality as described in~\cref{fig:main_result}.
The input and output dimensions of the projectors are configured to match the output dimension of the encoder and the input dimension of the decoder, respectively.
We train the projectors one epoch over the training set of the specific task in both pretraining and finetuning. 
In finetuning, we further set up early stopping with max patience equal to 500 steps, since the projectors quickly become convergent because of their small parameter size.
The details of training are listed in~\cref{tab:hyperparameters}.

==> tex/tables/projector_task_table.tex <==
\begin{table}
\centering
\caption{Projector Types and Modalities}
\label{tab:projector_type}
\begin{tabular}{>{\bfseries}l l} % Bold the first column
    \toprule
    Projector Type & Modality \\ 
    \midrule
    Linear         & Text, Numbers, Brain fMRI \\ 
    Non-linear     & Time-series, Graphs \\ 
    \bottomrule
\end{tabular}
\end{table}

==> tex/tables/sentiment_analysis_table.tex <==
\begin{table}[t]
    \centering
    \caption{We compare \methodlong with few-shot ICL and soft prompt tuning on the five sentiment analysis datasets. Details can be found in~\cref{sec:appendix_table_description}.
    %\jingbo{the pre-training results seem not stable and a little weak. Fine-tuning results might be only fair to compare with Soft Prompt? Shall we present other modality results first?}
    }
    \label{tab:sentiment_analysis}
    \small
    \begin{tabular}{l ccccc}
    \toprule
    \textbf{Method} & \textbf{Rotten Tomatoes} & \textbf{SST2} & \textbf{IMDB} & \textbf{Emotion} & \makecell{\textbf{Financial} \\ \textbf{Phrasebank}} \\
    \midrule
    \method (pretrained) & 80.60 & 78.90 & 95.04  & 41.20 & 60.72 \\
    Few-shot ICL      & 87.31 & 91.74 & 93.50 & 55.20 & 71.78 \\
    Soft prompt~\citep{li2021softprompt}  & \textbf{93.24} & 96.21 & 95.26  & 74.15 & 78.22 \\
    \method (finetuned)  & 88.80 & \textbf{98.16} & \textbf{97.28}  & \textbf{85.20} & \textbf{81.68} \\
    \bottomrule
    \end{tabular}
\end{table}


==> tex/tables/summarization_table.tex <==
\begin{table}[t]
    \centering
    \caption{We compare the performance of \methodlong, few-shot ICL, and soft prompt tuning across two text summarization datasets. 
    Details can be found in~\cref{sec:appendix_table_description}.
    }
    \label{tab:summarization}
    \small
    \begin{tabular}{l ccc}
    \toprule
    \textbf{Method} & \textbf{XSum} & \textbf{XLSum} \\
    \midrule
    \method (pretrained) & 15.25 & 15.89  \\
    Few-shot ICL &  19.53   & 19.41  \\
    Soft prompt  & 12.84 & 12.70 \\
    \method (finetuned)  & \textbf{20.08} & \textbf{20.49}  \\
    \bottomrule
    \end{tabular}
\end{table}

